Node Classification on Graphs with Few-Shot Novel Labels via Meta Transformed Network Embedding

We study the problem of node classification on graphs with few-shot novel labels, which has two distinctive properties: (1) There are novel labels to emerge in the graph; (2) The novel labels have only a few representative nodes for training a classifier. The study of this problem is instructive and corresponds to many applications such as recommendations for newly formed groups with only a few users in online social networks. To cope with this problem, we propose a novel Meta Transformed Network Embedding framework (MetaTNE), which consists of three modules: (1) A \emph{structural module} provides each node a latent representation according to the graph structure. (2) A \emph{meta-learning module} captures the relationships between the graph structure and the node labels as prior knowledge in a meta-learning manner. Additionally, we introduce an \emph{embedding transformation function} that remedies the deficiency of the straightforward use of meta-learning. Inherently, the meta-learned prior knowledge can be used to facilitate the learning of few-shot novel labels. (3) An \emph{optimization module} employs a simple yet effective scheduling strategy to train the above two modules with a balance between graph structure learning and meta-learning. Experiments on four real-world datasets show that MetaTNE brings a huge improvement over the state-of-the-art methods.

==> alg_procedure.tex <==

\begin{algorithm}[t]
\caption{The Optimization Procedure of \method{}}
\label{alg:procedure}
\begin{algorithmic}[1]
\REQUIRE
Graph $G$, total number of steps $N$
\ENSURE
The embedding matrix $\M{U}\in\mathbb{R}^{|V|\times M}$,
the function $Tr(\cdot)$
\STATE Randomly initialize $\M{U}$
and the parameters $\Theta$ of $Tr(\cdot)$
\FOR{$step=0$ \TO $N$}
\STATE Calculate the threshold $\tau$ via Eqn.~(\ref{eqn:threshold})
\STATE Draw a random number $r\sim \text{Uniform}(0,1)$
\IF[Optimize the structural module]{$r<\tau$}
\STATE Sample a batch of pairs $\{(v_i,v_j)|v_i\in\CV,v_j\in\CN(v_i)\}$
\STATE Update $\M{U}$
to optimize the objective function~(\ref{eqn:struc})
\ELSE[Optimize the meta-learning module]
\STATE Sample a batch of tasks $\CT_i$ from $\CY_{known}$
\FORALL{$\CT_i=(\CS_i,\CQ_i,y_i)$}
\FORALL{$v_q\in\CQ_i$}
\STATE Calculate the adapted embeddings
$\{\tilde{\V{u}}_{k,q}^{(i)}|v_k\in\CV_{\CS_i^m}\}$ and $\tilde{\V{u}}_{q,m}^{(i)}$,
where $m\in\{+,-\}$,
via Eqn.~(\ref{eqn:self-attention-query})~and~(\ref{eqn:self-attention-support})
\STATE Calculate the prototypes $\tilde{\V{c}}_{+,q}^{(i)}$ and $\tilde{\V{c}}_{-,q}^{(i)}$
via Eqn.~(\ref{eqn:new_proto})
\ENDFOR
\ENDFOR
\STATE Update $\M{U}$ and $\Theta$ to optimize the objective function~(\ref{obj:meta_adapt})
\ENDIF
\ENDFOR
\end{algorithmic}
\end{algorithm}


\begin{algorithm}[t]
\caption{Generalization to Few-Shot Novel Labels}
\label{alg:procedure_adapt}
\begin{algorithmic}[1]
\REQUIRE
The embedding matrix $\M{U}$,
the function $Tr(\cdot)$,
a novel label $y\in\CY_{novel}$,
associated positive support nodes $\CV_{\CS^{+}}$ and negative support nodes $\CV_{\CS^{-}}$,
query nodes $\CV_{\CQ}$
\ENSURE%
The predicted probability $\hat{\SL}_{v_q,y}$ for each query node $v_q$
\STATE Look up in $\M{U}$ to get the support and query embeddings $\mathbf{u}_{k}, \mathbf{u}_{q}$.
\FOR{$v_q$ in $\CV_{\CQ}$}
    \STATE Adapt $v_q$ together with $\CV_{\CS^{+}}$ according to Eqn. (\ref{eqn:adapt_sep}) and obtain adapted embeddings $\{\tilde{\V{u}}_{q,+}\}\cup\{\tilde{\V{u}}_{k,q}|v_k\in\CV_{\CS^{+}}\}$.
    \STATE Adapt $v_q$ together with $\CV_{\CS^{-}}$ according to Eqn. (\ref{eqn:adapt_sep}) and obtain adapted embeddings $\{\tilde{\V{u}}_{q,-}\}\cup\{\tilde{\V{u}}_{k,q}|v_k\in\CV_{\CS^{-}}\}$.
    \STATE Calculate the positive and negative prototypes $\tilde{\V{c}}_{m,q}, m\in\{+,-\}$ for classification according to Eqn. (\ref{eqn:new_proto}).
    \STATE Calculate the predicted probability with $\tilde{\V{c}}_{m,q}$ and $\tilde{\V{u}}_{q,m}$ according to Eqn. (\ref{eqn:new_prob_l}).
\ENDFOR




\end{algorithmic}
\end{algorithm}



==> figs/fig_example.tex <==
\begin{figure}[t]
\centering
\includegraphics[width=0.75\linewidth]{example}
\caption{
An example in social networks.
Each node represents a user and nodes are connected via friendship relationships.
The shaded regions indicate that different advertisements are distributed to the corresponding covered nodes,
and the symbols ``+'' and ``-'' indicate positive and negative feedback, respectively.
For a new advertisement that collects a few responses, we aim to infer other nodes' preferences
with the aid of prior knowledge from the graph structure and the results of previous advertisements 1 and 2.}
\label{fig:example}
\vspace{-15pt}
\end{figure}

==> figs/fig_schemes.tex <==
\begin{figure*}[!t]
\centering
\begin{subfigure}[b]{0.34\textwidth}
\includegraphics[width=\textwidth]{scheme_unsup}
\caption{Unsupervised Methods.}
\label{fig:scheme_unsup}
\end{subfigure}
\hfill
\begin{subfigure}[b]{0.01\textwidth}
\includegraphics[height=65pt]{vertical_line}
\vspace{15pt}
\end{subfigure}
\hfill
\begin{subfigure}[b]{0.24\textwidth}
\includegraphics[width=\textwidth]{scheme_semisup}
\vspace{0pt}
\caption{Semi-supervised Methods.}
\label{fig:scheme_semisup}
\end{subfigure}
\hfill
\begin{subfigure}[b]{0.01\textwidth}
\includegraphics[height=65pt]{vertical_line}
\vspace{15pt}
\end{subfigure}
\hfill
\begin{subfigure}[b]{0.36\textwidth}
\includegraphics[width=\textwidth]{scheme_our}
\caption{Our Method.}
\label{fig:scheme_our}
\end{subfigure}
\caption{
Learning schemes of different methods for \problem{}.
}
\label{fig:scheme}
\end{figure*}

==> tables/notation.tex <==
\begin{table}
\caption{Summary of notation}
\label{tab:notation}
\begin{tabular}{r@{\hspace{5\tabcolsep}}l}
\toprule
$\CG$ & undirected graph \\
$\CV$ & a set of nodes \\
$\CE$ & a set of edges \\
$\CY$ & \\
$\CY_{known}$ & \\
$\CY_{novel}$ & \\
$v_i$ & \\
$e_{ij}$ & \\
$y_j$ & \\
$\SL_{v_i,y_j}$ & \\
$\CD_{y_j}$ & \\
$\CD_{y_j,1}$ & \\
$\CD_{y_j,-1}$ & \\
\bottomrule
\end{tabular}
\end{table}
